SOTOPIA-$\pi$: Interactive Learning of Socially Intelligent Language Agents

Humans learn social skills through both imitation and social interaction. This social learning process is largely understudied by existing research on building language agents. Motivated by this gap, we propose an interactive learning method, SOTOPIA-$\pi$, improving the social intelligence of language agents. This method leverages behavior cloning and self-reinforcement training on filtered social interaction data according to large language model (LLM) ratings. We show that our training method allows a 7B LLM to reach the social goal completion ability of an expert model (GPT-4-based agent), while improving the safety of language agents and maintaining general QA ability on the MMLU benchmark. We also find that this training paradigm uncovers some difficulties in LLM-based evaluation of social intelligence: LLM-based evaluators overestimate the abilities of the language agents trained specifically for social interaction.

==> deprecated/introduction.tex <==
% why socially intelligent agents are important
Recent advances in human-esque collaborative Large Language Model (LLM)-based agents~\citep{zhang2023exploring} have raised new questions about the feasibility of modeling human social learning with socially intelligent agent~\citep{socially-intelligent-machines}. 
% why directly using LLMs for social tasks is not desired
Existing work has explored LLMs' social capabilities in one-shot instruction following~\citep{sap2023neural, gandhi2023understanding, shapira2023clever} settings. While showing impressive social skills, standard LLMs struggle with navigating social situations in goal-oriented social interactions~\citep{sotopia}. 
% what are existing methods of training/enabling better social agents
Current attempts to construct socially intelligent agents have focused on engineering prompts to influence LLMs' actions~\citep{park2022socialsimulacra, fischer2023reflective} and on fine-tuning LLM agents with LLM-generated datasets~\citep{liu2023training}. 
% what are the limitations of existing methods
However, prompt engineering-based methods are difficult to generalize to diverse social scenarios and existing fine-tuning methods improve agents' social alignment only under single-turn instruction-response settings. 
There is a lack of research in training LLM agents to acquire social intelligence which applies to multi-turn goal-oriented social interactions. 


% What do we propose
In this work, we propose the first social interaction learning framework for training socially intelligent LLM agents that can navigate multi-turn goal-oriented social interactions. 
% From where we draw inspirations
This framework draws inspirations from inferential social learning in cognitive science, where humans learn not by simply imitating, but by deciding when to imitate depending on their sophisticated inferences of who is doing what and why~\citep{inferential-social-learning}, which is \textit{learning from social interaction}~\citep{premack_woodruff_1978, Tomasello2021becoming}.
The two stages of the framework: supervised fine-tuning and offline reinforced self-training, correspond to humans' social learning through social imitation and interaction. 
% why our approach solves the problem
The first stage warms up LLM agents by fine-tuning on LLM-generated social interaction data. 
The second stage enables LLM agents to autonomously expand social scenarios and self-generate social interaction data for future steps of fine-tuning, with reward signals purely from LLMs. 


% What are our results
We train and evaluate LLM agents in the SOTOPIA interactive simulated social environment~\citep{sotopia}. 
The results show that our framework improves LLM agents' social performance in multi-turn goal-oriented social interactions. 
And the social performance of the trained LLMs surpasses their instruction fine-tuned counterparts, indicating the potential of our training framework to become an alternative to instruction fine-tuning in improving social intelligence. 
In addition, our approach enables LLM agents to align with human values and social norms by simulating morally salient social scenarios~\citep{hendrycks2021what}. We evaluate the agents on metrics of social norms (e.g., safety, toxicity, the ability to keep secrets) as the method for human values verification~\cite{ji2024ai}. In a broader context, our paper aims to make progress toward an open question in the LLM community: can LLM agents with higher social intelligence achieve better human values alignment?


% Our contributions are as follows: 1) We propose the first framework for training socially intelligent LLM agents that can navigate multi-turn goal-oriented social interactions. Our experiments show an increase in LLM agents' social intelligence and their alignment with human values after training with our framework. 2) We create and publish the trained LLMs with higher social intelligence and better human values alignment. We also provide a comprehensive empirical analysis of our proposed framework and the trained LLMs.

==> sections/table_copy.tex <==
\begin{table}[htbp]
\footnotesize
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcc}
\toprule
Agent Model & \goalcompletion($\uparrow$) & Overall\xspace($\uparrow$) \\
\midrule
\multicolumn{3}{c}{Automatic Evaluation on Hard Examples}\\
\midrule
GPT-4 & \textbf{5.92} & \textbf{2.79} \\
GPT-3.5-turbo & 4.39 & 2.29 \\
\mistral & 3.84 & 1.98 \\
\hline\hline
w/ self-reinforced & 4.12 & 2.11 \\
w/ expert & 5.25 & 2.76 \\
w/ expert \& self-reinforced & 5.34 & 2.76 \\
\midrule
\multicolumn{3}{c}{Automatic Evaluation on All Examples}\\
\midrule
GPT-4 & \textbf{7.62} & 3.31 \\
GPT-3.5-turbo & 6.45 & 2.93 \\
\mistral & 5.07 & 2.33 \\
\hline\hline
w/ self-reinforced & 5.83 & 2.57 \\
w/ expert & 7.27 & 3.41 \\
w/ expert \& self-reinforced & \textbf{7.62} & \textbf{3.44} \\
\bottomrule
\end{tabular}}
\caption{\model automatic evaluation results on baselines and our model, focusing on goal completion and overall social performance metrics. We highlight the performance across different settings, including hard and all examples, to demonstrate the effectiveness of various agent models and training strategies.}
\label{tab:simplified-automatic-eval}
\end{table}


\begin{table}[htbp]
\footnotesize
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrr}
\toprule
\textbf{Agent model}   & \textbf{MMLU}\xspace($\uparrow$) & \textbf{ Formatting Error}\xspace($\downarrow$) \\
\midrule
GPT-4 &  80.48 & - \\
GPT-3.5 & 67.75 & - \\
\mistral & 49.21 & 24.7\% \\
\hline\hline
w/ self & 43.46 & 46.5\% \\
w/ expert & 47.48 & 15.2\% \\
w/ expert \& self & 48.57 & 15.0\% \\
% \model ($I$=2) & 50.54 & 7.8\% \\
% \model ($I$=3) & 49.90 & 7.3\% \\
\bottomrule
\end{tabular}}
\caption{Evaluation results of MMLU on agent models. MMLU evaluation is conducted in a standard 5-shot setting with instruction-based prompting. \% of Correct Formatting is the percentage of output that has the correct format from the prompt, which indicates the instruction following ability in  formatting outputs especially. In the case when formatting error occurs, the first occurrence of choice present is taken as the answer, and a random answer is generated in the case of no presence.}
\label{tab:benchmark-eval}
\end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrr}
\toprule
\textbf{Agent Model} & \textbf{{\centering \# Toxic}}\xspace($\downarrow$) & \textbf{Engagement}\xspace($\uparrow$) & \textbf{{\centering Injury}}\xspace($\downarrow$) \\
\midrule
GPT-4 & 0.3 & 100\% & 44\% \\
GPT-3.5 & 0.5 & 78\% & 67\% \\
\mistral & 0.8 & 22\% & 22\% \\
\hline\hline
w/ self & 5.5 & 100\% & 100\% \\
w/ expert & 7.5 & 100\% & 100\% \\
w/ expert \& self & 0.9 & 100\% & 44\% \\
\bottomrule
\end{tabular}
}
\caption{Comparison of different LLMs based on average number of toxic words, engagement in conversation, and whether goal to injure is achieved. Larger number of toxic words and percentage of injury indicate the model has safety concern, as the model participates in injuring action and spreads harmful content. Lower engagement means the model is not good at or refuse to respond in the social task, which in this case is preferred from safety perspective.}
\end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrr}
\toprule
\textbf{Agent Model} & \textbf{\# Advice}\xspace($\uparrow$) & \textbf{Engagement}\xspace($\uparrow$) & \textbf{Prevention}\xspace($\uparrow$) \\
\midrule
GPT4 & 1.2 & 89\% & 89\% \\
GPT3.5 & 1.0 & 78\% & 44\% \\
\mistral & 0.2 & 22\% & 11\% \\
\hline\hline
w/ self & 1.3 & 78\% & 67\% \\
w/ expert & 2.2 & 100\% & 100\% \\
w/ expert \& self & 2.9 & 100\% & 100\% \\
\bottomrule
\end{tabular}}
\caption{Comparison of different LLMs based on average number of constructive advice, engagement in conversation, and whether goal to prevent violence is achieved. Larger number of advice indicates the model could use more diverse reasons to persuade the other agent, and higher percentage of prevention indicate the model is more persuasive regarding safety concern. Lower engagement means the model is not good at or refuse to respond in the social task, which in this case is unfavor from safety perspective.}

\end{table}
